Globally Optimal Symbolic Regression

In this study we introduce a new technique for symbolic regression that guarantees global optimality. This is achieved by formulating a mixed integer non-linear program (MINLP) whose solution is a symbolic mathematical expression of minimum complexity that explains the observations. We demonstrate our approach by rediscovering Kepler's law on planetary motion using exoplanet data and Galileo's pendulum periodicity equation using experimental data.

==> conclusions.tex <==
\newpage\section{Conclusions and Future Work}

The field of mathematical programming has evolved in the past 60 year dramatically, offering unmatched theoretical rigor, efficiency, and analyzability. 
Building upon these solids grounds, global optimality of the discovered models can be provably guaranteed. 
Provided that identifiability can becomes a problem, especially with limited dataset size, and / or in the presence of noise, additional guidance may facilitate quicker and more robust discovery of the underlying governing equations. 
An important characteristic of universal relations is the notion of invariancies. For an instance, translation and rotation invariance (reference system), symmetry, conservation, etc. Due to the great flexibility the proposed optimization-based 
framework offers, incorporation of implicit and explicit constraints, as well as meta-modeling preferences can be done seamlessly.  

 A key advantage of free-form discovery is the interpretability of the discovered equations which stand in contrast to fixed-form models. 
%These meta-level principles, ensures that the underlying 
%Fundamental law and relations, tend to be invariant. 
%, yet, generalizability is often attained, by 
The free-form model discovery optimization-based framework, can be applied to symbolic regression in the broader sense, thereby extending its utility to applications beyond model discovery. Future work would be to explore the utility of the approach for yet-to-be-discovered phenomenafor the advancement and acceleration of science discovery.

==> hybrid.tex <==
\subsection{Hybrid Data-Driven First-Principle Model Discovery}
%\footnote{\Leo{Referring to the subsection title: hybridization of what?}}
\textcolor{red}{It is evident that each approach
%\footnote{\Leo{Among which approaches?}} 
offers unique advantages while also involving innate shortcomings. The challenge is therefore, to find a way to hybridize the two approaches.
%\footnote{\Leo{So far, what I gathered from this text is that one approach is postulating a functional form aprioristically, and then use some fitting techniques to estimate the values of the parameters of the functional form from the data. I don't see any other approach.}}
This bring us to the fundamental modeling question as to whether one should
derive, or let the data drive?
%\footnote{\Leo{This sentence is unclear: one should derive what? and in what sense do data ``drive''? Or is this a mis-spelled word for ``derive''?}}  
At some level the two modeling approaches 
%\footnote{\Leo{This pronoun does not refer to any previous word in this paragraph. What are ``they''?}} 
are very similar, where they primarily differ by the choice of functional form and the level of automation associated with  the model formation.%\footnote{\Leo{``a different functional'' prefixes a singular, but ``forms'' is plural. I have not corrected it because ``and automation'' (a word which was never mentioned so far) makes the sentence unclear, so I wouldn't know how to correct it in order to clarify it.}} 
There is great synergy in combining the strengths of both. }%\footnote{\Leo{This sentence lacks a main verb; also, the sentence is vague: it was claimed above that two approaches (the second of which was not clearly stated) had advantages and disadvantages, but neither advantages nor disadvantages were actually stated.}}\\


==> mathModeling.tex <==
\subsection{First Principles and Data-driven Models}
The process of creating a mathematical model of the relationship between the inputs and outputs of a system involves choices which affect model complexity and realism. 
One must trade-off competing objectives such as accuracy, generalizability, 
robustness, functional complexity, scalability (computational complexity) and interpretability. Mathematical modeling techniques range from a first-principles approach based on fundamental laws to empirically learned data-driven models in statistics and machine learning. 

 A first-principles approach was the historical norm before the computing era, and usually requires significant domain expertise.
Recently, there has been a lot of progress in the automatic derivation of models in the form of data-driven approaches.
Such approaches typically prescribe a functional form for the relationship between the inputs and outputs and then use the data to find the parameters that completely define the function.
As an example, in linear regression one assumes a linear relationship and then one solves a least-squares problem to find the coefficients defining the linear relationship.
Thus, prescribing a linear functional form also leads to a computationally tractable solution approach. Of course, if the output does not linearly depend on data, the model can be quite inaccurate.
More general models (such as polynomials, which can yield an arbitrarily accurate model as they are dense in the set of continuous functions) usually require more data.
Such models can be effective when (i) limited domain expertise is available, (ii) a lot of data is available, and (iii) the available data is representative of all system states.

Selecting a functional form a priori thus has many drawbacks: one with few parameters may be too inaccurate; one with too many parameters may yield an accurate model but may need a lot of data, limited generalizabilty, and yield limited interpretational insight. 

